Variational Quantum Simulations of Finite-Temperature Dynamical Properties via Thermofield Dynamics

The recent advancement of quantum computer hardware offers the potential to simulate quantum many-body systems beyond the capability of its classical counterparts. However, most current works focus on simulating the ground-state properties or pure-state quantum dynamics of quantum systems. Finite-temperature physics are much less explored, and existing literature mainly consider equilibrium properties. Here we present a variational quantum simulation protocol based on the thermofield dynamics formalism to simulate the dynamical and non-equilibrium finite-temperature properties of quantum systems with near-term quantum computers. Compared to previous approaches in computing the equilibrium dynamical properties, our approach does not require the computationally expensive initial state sampling. More importantly, our approach is capable of simulating non-equilibrium phenomena which have not been previously explored with quantum computers. Numerical simulations of molecular absorption spectrum and spin quenched dynamics affirm the capability of our method.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> preamble.tex <==
\usepackage{graphicx,graphics,epsfig,subfigure,times,bm,bbm,amssymb,amsmath,amsfonts,amsthm,mathrsfs,MnSymbol}
\usepackage[matrix,frame,arrow]{xypic}
\usepackage[normalem]{ulem}
\usepackage{slashed}
%\usepackage[c]{hyperref}
\usepackage{color}
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}
\definecolor{darkblue}{rgb}{0.0,0.0,0.3}
%\usepackage[pdftex]{color}
%\usepackage[hidelinks]{hyperref}
\usepackage[colorlinks=true,
            linkcolor=red,
            urlcolor= darkblue,
            citecolor=blue]{hyperref}
%\usepackage{natbib}
%\usepackage{braket}%Dirac Notation in QM

\usepackage{enumerate}
\usepackage{epstopdf}
%\usepackage{pdfsync}
\usepackage{relsize}

\hyphenpenalty = 900
\linespread{0.956}

%\input{Qcircuit.tex}

\newtheorem{definitionenv}{Definition}
\newtheorem{remarkenv}[definitionenv]{Remark}
\newenvironment{remark}{\begin{remarkenv}\rm}{\end{remarkenv}}

\newtheorem{exampleenv}{Example}
\newenvironment{example}{\begin{exampleenv}\rm}{\end{exampleenv}}


\newtheorem{thm}{Theorem}
\newtheorem{mydef}{Definition}
\newtheorem{col}{Corollary}

\newtheorem{mytheorem}{Theorem}
\newtheorem{mylemma}{Lemma}
\newtheorem{mycorollary}{Corollary}
\newtheorem{myproposition}{Proposition}

\newcommand{\msf}{\mathsf}
\newcommand{\mrm}{\mathrm}
\newcommand{\mbf}{\mathbf}
\newcommand{\mbb}{\mathbb}
\newcommand{\mcal}{\mathcal}




\newcommand{\bes} {\begin{subequations}}
\newcommand{\ees} {\end{subequations}}
\newcommand{\bea} {\begin{eqnarray}}
\newcommand{\eea} {\end{eqnarray}}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{black}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}

\newcommand{\ph}{\ensuremath{\varphi}}
\newcommand{\eps}{\ensuremath{\varepsilon}} %"nice" epsilon
\newcommand{\prima}[1]{\ensuremath{#1^\prime}} %add a prime to something
\newcommand{\R}{\ensuremath{\mathbb{R}}} %real numbers
\newcommand{\C}{\ensuremath{\mathbb{C}}} %complex numebrs
\newcommand{\Q}{\ensuremath{\mathbb{Q}}} %rational numbers
\newcommand{\Z}{\ensuremath{\mathbb{Z}}} %integers
\newcommand{\N}{\ensuremath{\mathbb{N}}} %natural numbers
\newcommand{\e}{\ensuremath{{e}}} %e:=lim_{n\to\infty}(1+1/n)^n
\newcommand{\ii}{\ensuremath{{i}}}%i:=\sqrt{-1}
\newcommand{\abs}[1]{\ensuremath{\left|#1\right|}} %absolute value
\newcommand{\norm}[1]{\ensuremath{\left\|#1\right\|}} %norm
\newcommand{\opU}{\ensuremath{{{U}}}}
\newcommand{\opH}{\ensuremath{{{H}}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\dfsh}{\tilde{\mathcal{H}}}
\newcommand{\wt}[1]{\mathrm{wt}(#1)}
\newcommand{\eeq}{\end{equation}}

\newcommand{\upi}{\mathrm{i}}
\newcommand{\upe}{\mathrm{e}}
\newcommand{\upd}{\mathrm{d}}
\newcommand{\Tr}{\mathrm{Tr}}
\newcommand{\ignore}[1]{}
\newcommand{\mc}[1]{\mathcal{#1}}

%Greek Letters
\def\a{\alpha}
\def\b{\beta}
\def\g{\gamma}
\def\d{\delta}
\def\e{\epsilon}
\def\ve{\varepsilon}
\def\z{\zeta}
\def\h{\eta}
\def\t{\theta}
%\def\i{\iota}
\def\k{\kappa}
%\def\l{\lambda}
\def\m{\mu}
\def\n{\nu}
\def\x{\xi}
\def\p{\pi}
%\def\r{\rho}
\def\s{\sigma}
\def\ta{\tau}
\def\u{\upsilon}
\def\ph{\varphi}
\def\c{\chi}
\def\ps{\psi}
\def\o{\omega}

\def\G{\Gamma}
\def\D{\Delta}
\def\T{\Theta}
\def\Lam{\Lambda}
\def\X{\Xi}
\def\P{\Pi}
\def\S{\Sigma}
\def\U{\Upsilon}
\def\Ph{\Phi}
\def\Ps{\Psi}
\def\O{\Omega}

%Some helpful quantum shortcuts
\def\ox{\otimes}
\def\>{\rangle}
\def\<{\langle}
\def\Tr{\mathrm{Tr}}
\def\Pr{\mathrm{Pr}}

\newcommand{\ketbra}[1]{|{#1}\>\<#1|}
\newcommand{\bracket}[1]{\<{#1}|{#1}\>}
\newcommand{\bk}[2]{\<{#1}|{#2}\>}
\newcommand{\ketb}[2]{|{#1}\>\<#2|}
\newcommand{\ketbsub}[3]{|{#1}\>_{#3}\<#2|}
\newcommand{\ident}{\mathbb{I}}
\newcommand{\bra}[1]{\langle#1|}
\newcommand{\ket}[1]{|#1\rangle}


\newcommand{\opI}{\ensuremath{{{I}}}}
\newcommand{\opA}{\ensuremath{{{A}}}}
\newcommand{\opB}{\ensuremath{{{B}}}}
\newcommand{\opX}{\ensuremath{{{X}}}}
\newcommand{\opY}{\ensuremath{{{Y}}}}
\newcommand{\opZ}{\ensuremath{{{Z}}}}
\newcommand{\opS}{\ensuremath{{{S}}}}
\newcommand{\ee}{\ensuremath{{e}}} %e:=lim_{n\to\infty}(1+1/n)^n


%\newcommand{\cC}{\mathcal{C}}

%These last ones are due to florjanc@usc.edu, please email me if they conflict with something and you'd like me to revise what I've written to not use them.
\def\lp{\left(}
\def\rp{\right)}
\def\ls{\left[}
\def\rs{\right]}
\def\lb{\left\{}
\def\rb{\right\}}

%By muthukri@usc.edu

\def\dgr{\dagger}

%from Ching-yi
\newcommand{\sfA}{\textsf{A}}
\newcommand{\sfB}{\textsf{B}}
\newcommand{\sfC}{\textsf{C}}
\newcommand{\sfD}{\textsf{D}}
\newcommand{\sfE}{\textsf{E}}
\newcommand{\sfF}{\textsf{F}}
\newcommand{\sfG}{\textsf{G}}
\newcommand{\sfH}{\textsf{H}}
\newcommand{\sfI}{\textsf{I}}
\newcommand{\sfM}{\textsf{M}}
%
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
%\newcommand{\cH}{\mathcal{H}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
%\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}

\newcommand{\rmark}[1]{{\color{red} #1}}
\newcommand{\bmark}[1]{{\color{blue} #1}}
\newcommand{\step}{\tau} %% to replace \mathcal{T}
\DeclareMathOperator*{\bigcdot}{\raisebox{0pt}[\ht\dotbox][\dp\dotbox]{\(\boldsymbol{\cdot}\)}}
